Fast and Work-Optimal Parallel Algorithms for Predicate Detection

Recently, the predicate detection problem was shown to be in the parallel complexity class NC. In this paper, we give the first work-optimal parallel algorithm to solve the predicate detection problem on a distributed computation with $n$ processes and at most $m$ states per process. The previous best known parallel predicate detection algorithm, ParallelCut, has time complexity $O(\log mn)$ and work complexity $O(m^3n^3\log mn)$. We give two algorithms, a deterministic algorithm with time complexity $O(mn)$ and work complexity $O(mn^2)$, and a randomized algorithm with time complexity $(mn)^{1/2 + o(1)}$ and work complexity $\tilde{O}(mn^2)$. Furthermore, our algorithms improve upon the space complexity of ParallelCut. Both of our algorithms have space complexity $O(mn^2)$ whereas ParallelCut has space complexity $O(m^2n^2)$.

==> AlgDescrPred.tex <==
% % !TEX root = garg-pred.tex
% % !TEX root = disc18.tex
% \subsection{The ParallelCut Algorithm}

% %Before we begin to describe the algorithm it is important we establish some definitions and how we will denote various objects throughout the paper. 
% %We will refer to the $jth$ state on the $ith$ process as the tuple $(i,j)$. We use this tuple notation because we index our states in our array-based data structures using $array[i][j] = (i,j)$. This makes it convenient to interchangeably refer to states in the data structures as well as the states in the models we use. 

% %We use both conventions becasue in some cases we want to refer to just the process index or just the state index. For this, the first denotation, $P_i.S[j]$ is more convenient. However, we we interact with the matrixes $R$ and $RT$, as well as the arrays $valid$, $bestValid$, and $Cut$, it is convenient to use the tuple denotation. 

% %Throughout the paper, we will be using Lamport's $happened-before$ relation to represent causality between states. A state $e$ happens before another state $f$ when $e$'s vector clock value is less than that of $f$'s. Thus, $e \ra f $ iff $VC[e] < VC[f]$. 
% We now review the \textit{ParallelCut} Algorithm. The key technique is computing a {\em state rejection  graph}.
% The state rejection graph is a directed graph with all local states as vertices of the graph.
% Let state $j$ on process $i$ be denoted as $(i,j)$.
% The state rejection graph puts a rejection edge from the state $(i,j)$ to $(i',j')$ if the rejection of state $(i,j)$ as a possible component of the
% consistent cut implies that the state $(i',j')$ will also be rejected.

% \begin{figure}[htbp]
% %\vspace*{-0.3in}
% \begin{center}
% %\includegraphics[height=2.5in]{exampleVecClockmodel.pdf}
% \includegraphics[height=2.4in]{example3.pdf}
% \caption{\label{fig:reject} State Rejection Graph of a computation shown in dashed arrows }
% \end{center}
% %\vspace*{-0.2in}
% \end{figure}

% In Fig. \ref{fig:reject} we show the state rejection graph of the computation in Fig. \ref{fig:model}.\\


% Intuitively, the state rejection graph gives us the relation that if state $s$ is not in any consistent cut and there is an edge from $s$ to another state $s'$, then $s'$ will not be a part of any consistent cut either. %So, we can compute the first few states that are rejected and find all states reachable from these initially rejected states. These states never appear in any consistent cut of the computation. 
% %by using reachability from $F$, we can compute all the states that never appear in any consistent cut. 
% Crucially, the \textit{rejection} of state $s$ implies the rejection of state $s'$ but \textit{also} implies the rejection of \textit{all} states that happened-before state $s'$. We will see the importance of this fact throughout the explanation of the algorithm.\\

% Informally, the algorithm proceeds as follows. We find out which states cannot be included in the first possible consistent cut. These states make up the set $F$. We then follow the rejection edges to all vertices reachable by some node in $F$ and {\em remove} these vertices from the graph. These vertices can never be a part of any consistent cut. Lastly, we find the first remaining vertex on each process and all such states make up the minimum consistent cut. If there is any process that has no state remaining, we know there is no consistent cut for which $B$ evaluates to true. In this figure, if we remove all vertices in $F$ and any vertex reachable from these vertices using the red state rejection arrows, we see that the first consistent cut is the fourth state on $P_1$,the second state on $P_2$ and the third state on $P_3$.


% The input to the algorithm is a two-dimensional array of vector clocks. The following explanation of the {\em ParallelCut} algorithm is taken from \cite{Garg:2019}. \\
% %We call the representation of the computation the computation graph.
% %and our motivations behind certain design choices in the algorithm. 


% \noindent
% {\bf Step 1}:
% We first create $F$, the set of all initially rejected states.  Let $I$ be the global state consisting of each processor's first local state, i.e., 
% $ I = \{ (i,1) ~|~ i \in 1..n \} .$ If there are no dependencies between any of these states, we have already reached the first consistent global state. Else, if there is a dependency from one of these states to another, we reject whichever state happened-before the other and add it to $F$.
% We represent the set $F$ by a boolean bit array of size $n$ that is indexed by processor. 
% %Thus, $F[i] = 1$ iff $(i,1)$ is in $F$. 
% %We initialize the bit array with zeroes, i.e., 
% $F$ is initially empty. Then, we set $F[i]$ to $1$ whenever there exists a state $(j,1)$ such that $(j,1) \ra (i,1)$.
% %is the top choiceof $m'$ and $w$ prefers $m'$ to $m$.
% % Formally, 
% %\[ \forall i \in 1 \dots n: F[i] = 1 \equiv \exists j: (i,1) \ra (j,1)  \]

% %To demonstrate the construction of this graph as well as the procedure of the entire algorithm we present an example instance of a distribtued computation as a two-dimensional array of vector clocks. We will use this set of inputs for our entire explanation of the algorithm in the paper. Given the following input, our algorithm creates the corresponding state rejection graph. 

% %$$\textit {FIGURE HERE OF LIKE PROCESSES W ARROWS AND EVENTS LABELED WITH VECTOR CLOCKS}$$

% %In the first round , we assume that all processes chose their first local state in {\em parallel}. 
% %If any state $s \in I$ that is the first for any given process $\textit {happened before}$ another state $s' \in I$, then $s$ is added to $F$. 
% %%Informally, if any state in the first global state has happened-before any other state in the first global state, than all the states that happened-before the most recent state(s) in the first global state are added to $F$. 
% %%

% %If any woman $w$ has been proposed by a man $m'$ in the first round, then all proposals $(m,w)$ such that$rank[w][m] > rank[w][m']$ are added to $F$. In other words, all men $m$ who are less preferred than $m'$ are considered rejected.It is important to note that $m$ may not have yet made a proposal to the woman $w$, but it is guaranteed to be rejected whenever it is made.

% %To create $F$, 
% %we check if there are any two proposals $p = (m,w)$ and $ p' = (m',w')$ such that $mpref[m][i] = mpref[m'][1]$. In other words, we are seeing if any man $m'$ proposes to any other man $m$'s first choice. If so, we refer to $rank$ and add the man with the lower preference to $F$. Formally, let $w = mpref[m][i]$ and $w' = mpref[m'][1]$, and if $rank[w][m]$ $>$ $rank[w][m']$, then $F[(m,w)] = 1$. 

% %Our motivation for creating $F$ is that we know states in $F$ are guaranteed to be rejected in the first round. Then, once we create the state rejection graph, we can deduce what states  will be rejected after the states in $F$ are rejected. 

% This step can be done in $O(1)$ time in parallel with $O(n^2)$ work by using a separate processor for each value of $i$ and $j$.
% %. Since we have $n^6$ processors, we can compute the $for$ loop of three variables $m, i$ and $m'$ in parallel. Every operation under each combination of $m, i$ and $m'$ is done in constant time. Thus, this entire step takes constant time.

% %In Fig. \ref{fig:model},  $I =  \{ \langle 1,0,0 \rangle, \langle1,1,0\rangle, \langle0,0,1\rangle \}$. Among these elements, $\langle1,0,0\rangle \ra \langle1,1,0\rangle$. Thus, $\langle1,0,0\rangle \in F$. 

% %Informally, we have all men concurrently propose to their first choice. Now, there are two cases we must address. The first case is that all men have proposed to their first choice woman and no two men have the same first choice woman. Then, we have already reached the man-optimal stable matching. The second case is that there is an overlap between at least two men. At this point, we refer to $wpref$ 

% \noindent
% {\bf Step 2:}
% %
% %We define the state rejection graph as $G_P = (P, E)$. There exists an edge $e ~\in E$ from any state $s$ to another state $t$ if and only if:
% %
% %$$ t \ra succ(s) $$ 
% % 
% In step two, we create the state rejection graph represented as an adjacency matrix.  We define a new two-dimensional array called $R$, which is of size $mn \times mn$, where each row and each column represents a different state. In this directed graph, there is an edge from state $(i,j)$ to another state $(i',j')$ only if we know that once state $(i,j)$ is rejected, state $(i',j')$ will also be rejected. 
% In the adjacency matrix $R$, this is represented as $R[(i,j),(i',j')] = 1$. Additionally, we make the diagonal of the matrix all $1$'s. 
% %This means that the relation is reflexive once we create the matrix. %Formally, for every $(i,j)$, $R[(i,j),(i,j)] = 1$. 
% We show that creating this boolean matrix can be done in constant time. First, 
% %we separately set every location of the form $R[(m,w),(m,w)] = 1$. To do this, we carry out a $for$ loops of two variables $m$ and $w$ in parallel. We can do this in constant time because there are only $n$ indices of the form $R[(m,w),(m,w)]$. Thus, 
% setting the diagonal to all 1's in $R$ takes constant time. We now discuss how off-diagonal entries are set. This is a crucial step in our algorithm.
% Suppose that a state $(i,j)$ is rejected. We know that the processor will advance to the next state.
% % $m$ is going to make proposal to his next choice.
% Then, the next choice for that processor is $(i,j+1)$.
% Thus, the rejection of $(i,j)$ would lead to the rejection of all states $(i',j')$ where $(i',j') ~\ra (i,j+1)$.
% Formally,
% \[ R[(i,j),(i',j')] = 1 \equiv
%  (i',j') \ra (i, j+1)
%   \]
 
% By using a separate processor for each tuple $(i, j, i', j')$, we can set $R$ in $O(1)$ time and $O(m^{2}n^{2})$ work. We represent the state rejection graph as a boolean matrix so that we can compute the transitive closure of this graph by doing matrix multiplications. 
% %By repeated squaring $\log n$ matrix multiplications are required.

% %In our example problem, to create $R$, informally, we have every state check for incoming $happened-before$ arrows to its successor. If there are any incoming arrows, we add a rejection edge to the digraph. Doing this in parallel for every state creates $R$. 
% %
% %$$ \textit{ FIGURE HERE OF BOOLEAN MATRIX.} $$


% %Once we've set the diagonals of $R$, we have to set all other entries. Now, we have a $for$ loop of three variables $m, i$ and $m'$. This for loop, sequentially would take $O(n^3)$ time. However, since we have $n^6$ processors, this loop will be done in the same timestep by $n^3$ processors. Additionally, the $if$ statement under the $for$ loop will also be done on constant time. Thus, this entire step takes $O(1)$ time. 

% % i think there needs to be more discussion of why/how proposals are set to 1 in R. I only talked about time complexity and not well. I need to look over secction 3 alot.

% \noindent
% {\bf Step 3:}
% In step three, we take the transitive closure of $R$. The transitive closure of $R$ is also represented as an adjacency matrix $RT$.
% %Formally, %$RT$ satisfies that
% %for all  $i,i' \in 1 \dots n$  and $j, j' \in 1 \dots m:$
% %$ RT[(i,j)(i',j')] = 1$ iff  there exists a $k \in 1 \dots mn: R^{k}[(i,j)(i',j')] = 1.$
%  It is well known that the transitive closure for any directed graph with $|V|$ vertices can be computed in $O(\log |V|)$ time using $O(|V|^3 \log |V|)$ work on the common CRCW PRAM
%  \cite{jaja1992introduction}. Since our graph has $O(mn)$ vertices, this step takes $O(\log mn)$ time using $O(n^{3}m^{3} \log mn)$ operations on the CRCW PRAM.
%  This is the only step in our algorithm that takes more than $O(1)$ time. 
%  %$$ \textit{ FIGURE HERE OF  SAME BOOLEAN MATRIX W CLOSURE.} $$
 
% % If we look at the boolean matrix, we can view the transitive closure of of $R$ as applying matrix multiplications to $R$ to get $RT$. Again, since we only care about $\langle 1,0,0\rangle$, since it is in $F$, we only look at the $1's$ in the row for $<1,0,0>$. In the matrix, state $<1,0,0>$ would be represented as state $(1,1)$ since it is the first state on the first process. Again, in the matrix $RT$, we will see that there will be $1's$ under states $ (3,1), (2,1), (1,2), (1,3), (3,1)$.
 
%  \noindent
% {\bf Step 4:}
% In step four, we use both $F$ and $RT$ to determine which states will not be part of the first consistent global state. To do this, we create a new two-dimensional array called $valid[1 \dots n][1 \dots m]$ where each entry is a value of $0 \dots 1$. We initialize every entry in $valid$ to $1$ in $O(1)$ time with $O(mn)$ work.  
% The algorithm sets rejected states in $valid$ with a $0$. 
% %simply hold the value $j$ for the $jth$ state along any process 
%  %be a copy of $mpref$ in $O(1)$ time with $O(n^2)$ work.  
% %Now that we have initialized $valid$, we have to somehow denote which states are going to be rejected. We do this by overwriting rejected states in $valid$ with a $0$. 
% %Since 0 is out of bounds for the preference, it is easy to tell which proposal will be each man's first man-optimal pairing. 
% %To know which states will be set to $0$, we refer to both $RT$ and $F$. 
% We use $F$ and $RT$ for this purpose.
% For all possible values of  $i, j, i',$ and $j'$, in parallel, we check to see if a state $(i,j)$ is an element of $F$ and if there is an edge from $(i,j)$ to another state $ (i',j')$. 
% If the two states $(i,j)$ and $(i',j')$ fit this criteria, then we set $valid[i'][j']$ to $0$. In other words, if a state $(i,j)$ is initially rejected, and there is an edge from $(i,j)$ to $(i',j')$ in $RT$, then we know the state $(i',j')$ will also be rejected. 
% %Formally, for all $ i \in 1 \dots n, j \in 1 \dots m$:
% %\[ valid[i][j] = 0 \equiv \exists i': F[(i') = 1 \wedge RT[(i',1), (i, j)] = 1 \]

% %If $valid[i][j]$ is not changed then it must contain the initialized value, i.e.,
% %
% %\[ \forall i \in 1 \dots n, j \in 1 \dots m: valid[i][j] \neq 0 \Ra valid[i][j] = 1 \]
% %

% %constant time. Initializing $valid$ to be a copy of $mpref$ has only $n^2$ indices which is strictly less than the amount of processors we have. Then our next for loops spans $n^4$ indices which is also strictly less than the $n^6$ processors our algorithm requires. Thus, both of these loops and the operations done in these loops can be computed in $O(1)$ time. The first loop will take $O(n^2)$ operations on
% %
% % _________ 
% %PRAM. Also discuss other PRAMs. The second loop takes....... finish this part w dad.

% %dont know how to caluclate work on diff pram models here lmao mah b

% %In our example, we can view the transitive closure in two ways. This can either be seen as adding rejection edges in the digraph $R$. It can also be seen as performing matrix multiplication to the data structure version, the two-dimensional boolean matrix, of $R$. 
% %
% This step can also be done in $O(1)$ time and $O(m^{2}n^{2})$ work.
% In our example, we compute the states reachable by $\langle 1,0,0\rangle$. In our example, states $\{ \langle 0,0,1\rangle, \langle 1,1,0\rangle, \langle 2,0,\newline 1\rangle, \langle3 ,0,1\rangle \}$ are all reachable by $\langle1,0,0\rangle$ by following
% one or more rejection edges. 
% %For example, rejection of $<1,0,0>$ implies that $P_2$ has to be at least in the state $<2,0,1>$ which in turn implies that
% %$<0,0,1>$ will be rejected.
% Thus, we mark the states $ (1,1), (2,1), (3,1), (1,2), (1,3)$ with $0's$ in $valid$. 


% %If we only look at the model, we only care about the states in $F$ so we will only look at the states that are reachable by $<1,0,0>$. There is a $1$ from $<1,0,0>$ to $<0,0,1$ in $R$, so now we must look at what states are reachable from $<0,0,1>$ in $R$. 
% %Once we do this for all states, we will see that the states $\left\{ <0,0,1>, <1,1,0>, <3,0,2>, <0,0,2> \right\}$ are all reachable by $<1,0,0>$. 
% %
% %In our example, the construction of $valid$ can be seen as a two-dimensional array representation of the computation where $valid[I][j] = j$ represents the $jth$ state on the $ith$ process. We remove all the states reachable by state $(1,1)$ in $RT$. 
% %Thus, we replace the states $ (3,1), (2,1), (1,2), (1,3), (3,1)$ with $0's$ in $valid$. 
% %

% %\paragraph{Step 5:}
% %In step five, we create a new data structure called $firstValid$ where all states that are not in the first consistent cut are replaced with a $0$. It is important to note that $firstValid$ is different from $valid$. $Valid$ replaces all invalid states with a $0$, but $firstValid$ will only have non-zero values associated with the states that compose the first consistent global state. To do this, we first copy $valid$ into $firstValid$. 
% %%We copy $valid$ into $bestValid$ by using a $for$ loop of two variables, 
% %%$m$ and $i$ from $1 \dots n$, and assigning $bestValid[m][i] := valid[m][i]$. 
% %Next, we have to get rid of all states that are not in the first consistent cut. Trivially, each processor's state that is in the first consistent cut is it's first available valid state. 
% %For every processor, the algorithm reads $valid$ from left to right and chooses the first non-zero state and sets all other states in $bestValid$ to $0$. 
% %Formally,
% %\[ \forall m,i: firstValid[m][i] \neq 0 \equiv (firstValid[m][i] = valid[m][i]) \wedge (\forall j: j < i: valid[m][j] = 0) \]
% %Since $firstValid$ is initialized using $valid$ all zero entries stay the same, i.e.,
% %
% %\[ \forall m,i: valid[m][i] = 0 \Ra (firstValid[m][i] = 0)  \]
% %
% %%To do this, we traverse through $valid$ and check, for every man, the first proposal such that every proposal before it has a value of $0$. Intuitively, each man's man-optimal pair is his first available valid pair. The reader can also think about this as, for every man, reading $valid$ from left to right and choosing the first non-zero proposal and setting all other proposals in $bestValid$ to $0$. 
% %This step can be done in $O(1)$ time and $O(n^3)$ work.
% %%This step can be done in constant time. Our first loop copies $valid $ into $bestValid$. This process covers $n^2$ indices which is less than the $n^6$ processors we require. Thus, this $for$ loop can be completed in constant time. The next $for$ loop covers $n^3$ indices as we traverse$n^2$ indices for $n$ men. However, this too can be done in constant time since we have $n^6$ processors.
% %
% %In $firstValid$, we simply remove all the states that are not in the first consistent cut. Thus, from our example, we will remove states $(1,4), (2,3), (2,4), (3,4)$ from valid. We copy $valid$ into $firstValid$ and then replace the removed states with the value $0$. This way, there only exists one set of non-zero values which represent the first consistent global state. 

% \noindent
% {\bf Step 5:}
% In step five, we traverse $valid$ and construct the set of states that form the consistent global state in a new array called $cut$ where $cut[i] = j$ signifies that the tuple $(i,j)$ is
% a part of the consistent global state. To do this, for every process, in parallel, we simply search for the first entry which is nonzero and either it is the first entry or
% the entry prior to it is zero.

% %Formally, 
% %%$for$ all $i$ in 1 \dots n and $j$ in $1 \dots m$, if $firstValid[i][j] \neq 0$, then $cut[i] := firstValid[i][j]$.
% %$\forall i,j: (valid[i][j] \neq 0) \wedge ((j=1) \vee (valid[i][j-1] =0)) \equiv  (cut[i] = valid[i][j]).$\\
% % Again, intuiutively, this is the same as, for every man, reading from left to right and assigning each man to his only non-zero value associated woman. 
 
% In our example, we can easily see that the first consistent global state is the set $cut = \{ (1,4), (2,2), (3,2)\}$. 
% This step can be done in $O(1)$ time and $O(nm)$ work.
% % Again, this step can be completed in constant, $O(1)$, time. For all $n$ men, we traverse $n$ proposals. Thus, this step covers $n^2$ indices, which is less than the $n^6$ processors we require. 

% %Our algorithm creates a new data structure with different properties at each step. We first create a set to represent the initial forbidden states $F$. Then, we create a matrix $R$ to represent a graph which shows dependencies between states. We then create $RT$ which is the transitive closure of $R$. Lastly, we create two data structures, one to label which states are $valid$ and the other to determine the first $cut$.
% %It is interesting to note that this algorithm can be viewed as just the creation of a new data structure with different properties at each step. 

% %Table \ref{fig:TW} summarizes the time and work complexity of each step. 
% Thus, the entire algorithm takes $O(\log mn)$ time and $O(m^3n^3 \log mn)$ work on a
% common CRCW PRAM.



% {\bf Remark:} Note that the algorithm to detect a conjunctive predicate can be used to detect a global predicate in Disjunctive Normal Form.
% A predicate is  in Disjunctive Normal Form (DNF) if it is expressed as a disjunction of $k$ pure conjunctions. To detect a predicate in this form it is sufficient to detect each conjunction in parallel. 


% %On a CRCW PRAM, it is easy to determine if any
% %conjunction is true in $O(1)$ time.

% %$for$ every 
% %\subsetion{Remarks on the Algorithm}



% %Since we have $n^4$ processors, and there are a total of $n^4$ entries in the $R$ matrix, we can assign each proposal tuple of the form $((m,w),(m',w'))$ to a unique processor which corresponds to a different, unique entry in $R$. Then, each processor  ....... i don't know how to explain that this can be done in constant time.

% %Now, since we want to be able to compute reachability, we have to take the transitive closure of $R$. 

% %shows the relation where if some proposal $p$ gets rejected 

% %if some proposal $p$ to point to another proposal $p'$ in  $R$, it must fit the following definition.



==> DetConjPred.tex <==
\subsection{Detecting Conjunctive Predicates in Parallel}
\label{sec:conj}
In this subsection we outline some key properties used in the intuition behind the \textit{ParallelCut} algorithm. \textit{ParallelCut} detects a conjunctive predicate of the form $B = l_1 \wedge l_2 \wedge \dots \wedge l_n$.
To detect $B$, we need to determine if there exists a consistent global state $G$ such that
$B$ is true in $G$. Note that given a computation on $n$ processes each with $m$ states, there
can be as many as $m^n$ possible consistent global states. Therefore, enumerating and
checking the condition $B$ for all consistent global states is not feasible.
Since $B$ is conjunctive, it is easy to show \cite{GargWald:Unstable} that $B$ is true iff there exists a set of states $s_1, s_2, ..., s_n$ such that
(1) for all $i$, 
$s_i$ is a state on $P_i$, (2) for all $i$, $l_i$ is true on $s_i$ and (3) for all $i,j$: $s_i \| s_j$.
The \textit{ParallelCut} algorithm will either output such local states or guarantee that it is not possible to find them in the
computation.
When the global predicate $B$ is true, there may be multiple $G$ such that $B$ holds in $G$.
For conjunctive predicates $B$, it is known that there is a unique minimum global state $G$ that satisfies $B$
whenever $B$ is true in a computation \cite{ChaGar:DC}. 
We are interested in algorithms that return the minimum  $G$ that satisfies $B$.
The minimum $G$ corresponds to the smallest
counter-example to a programmer's understanding because $B$ typically represents the violation of a safety constraint.
%Our algorithms return the least global state $

%The \textit{ParallelCut} algorithm is based on the setting where the execution traces for all processes
%have been collected at one process. This setting is similar to the centralized algorithm where we have one checker process and $n$ application processes that are involved in detecting the predicate. Each process checks for local predicates during the computation and sends messages to the checker process whenever the local predicate becomes true \cite{GargWald:Unstable}.

%For example,
%in the centralized algorithm for conjunctive predicate detection, one process serves as a checker
%and collects the traces. 
%All other processes involved
%in detecting the WCP, referred to as application processes, 
%Each application process $P_i$
%check for local predicates during the computation.
%Each process $P_i$ also maintains the vector clock algorithm.
%Whenever the local predicate of a process becomes true for the {\em first} time since the
%most recently sent message (or the beginning of the trace), it
%generates a debug message containing
%its local timestamp vector and sends it to the checker process \cite{GargWald:Unstable}.

%The checker process uses queues of incoming messages to hold incoming local snapshots
%from application processes.
%For convenience, we require that messages from an individual process be
%received in FIFO order. If the underlying system is non-FIFO, then sequence numbers can be attached with messages to ensure FIFO
%delivery.
%At the end of the 
%computation, the checker process has a sequence of local states from each process where its local predicate is true.
%We now review the parallel algorithm to detect $B$ on these traces presented in \cite{Garg:2019}.

%We abstract the message passing system as a set of $n$ FIFO queues, one
%for each process.  
%We use the notation $q[1 \ldots n]$ to label these
%queues in the algorithm.


